On Random Graph Properties

We consider 15 properties of labeled random graphs that are of interest in the graph-theoretical and the graph mining literature, such as clustering coefficients, centrality measures, spectral radius, degree assortativity, treedepth, treewidth, etc. We analyze relationships and correlations between these properties. Whereas for graphs on a small number of vertices we can exactly compute the average values and range for each property of interest, this becomes infeasible for larger graphs. We show that graphs generated by the \ErdosRenyi graph generator with $p = 1/2$ model well the underlying space of all labeled graphs with a fixed number of vertices. The later observation allows us to analyze properties and correlations between these properties for larger graphs. We then use linear and non-linear models to predict a given property based on the others and for each property, we find the most predictive subset. We experimentally show that pairs and triples of properties have high predictive power, making it possible to estimate computationally expensive to compute properties with ones for which there are efficient algorithms.

==> Exploring the Space of Labeled Graphs/classification_performance.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[b!]
\caption{Demonstration of the top 10 pairs (left table) and triples (right table) of graph properties that achieve the best accuracy scores according to Random Forest.}
\vspace{0.3cm}
\begin{tabular}{|l|l|l|l|l|}
\hline
Properties                  & RF    & LR & SVM     & NN               \\ \hline
GCC,  $\rho$              & \textbf{89.2\%} & 55.5\%             & 89.2\% & 77.3\%          \\ \hline
GCC, ASCC                          & \textbf{85.4\%} & 55.4\%             & 65.8\% & 67.4\%          \\ \hline
GCC, den                          & \textbf{82.1\%} & 53.7\%             & 81.4\% & 72.3\%          \\ \hline
GCC, APL                          & \textbf{81.8\%} & 50.8\%             & 61.6\% & 64.5\%          \\ \hline
GCC, $R_G$   & \textbf{81.8\%} & 55.0\%             & 81.5\% & 79.7\%          \\ \hline
GCC, r                            & \textbf{78.2\%} & 72.7\%             & 79.6\% & 81.3\%          \\ \hline
GCC, $C_C$     & \textbf{77.0\%} & 62.0\%             & 74.0\% & 74.6\%          \\ \hline
GCC,  $C_{ei}$ & \textbf{75.5\%} & 56.9\%             & 76.0\% & 71.3\%          \\ \hline
GCC, $C_e$          & 73.5\%          & 63.5\%             & \textbf{76.8}\% & 75.8\% \\ \hline
GCC, $C_B$        & \textbf{71.3\%
} & 51.0\%             & 62.4\% & 69.6\%          \\ \hline
\end{tabular}
\quad
\begin{tabular}{|l|l|l|l|l|}
\hline
Properties                                   & RF    & LR & SVM     & NN      \\ \hline
\scalebox{0.75}[1]{GCC, ASCC, $\rho$   }                      & \textbf{92.8\%} & 56.6\%             & 72.4\% & 88.1\% \\ \hline
\scalebox{0.75}[1]{GCC, ASCC, APL}                                     & \textbf{92.5\%} & 54.3\%             & 66.1\% & 62.4\% \\ \hline
\scalebox{0.75}[1]{GCC, ASCC, den   }                                   & \textbf{92.5\%} & 56.7\%             & 72.4\% & 76.3\% \\ \hline
\scalebox{0.75}[1]{GCC, APL, $\rho$}                        & \textbf{92.0\%} & 55.2\%             & 70.6\% & 80.6\% \\ \hline
\scalebox{0.75}[1]{GCC, ASCC, $R_G$}               & \textbf{91.9\%} & 57.4\%             & 75.7\% & 73.5\% \\ \hline
\scalebox{0.75}[1]{GCC, den, $\rho$}                       & \textbf{91.7\%} & 54.1\%             & 91.2\% & 82.2\% \\ \hline
\scalebox{0.75}[1]{GCC, $C_e$, $\rho$}            & \textbf{90.9\%} & 63.9\%             & 82.3\% & 82.0\% \\ \hline
\scalebox{0.75}[1]{GCC, den, $R_G$  }           & \textbf{90.5\%} & 56.4\%             & 85.6\% & 75.5\% \\ \hline
\scalebox{0.75}[1]{GCC, r, $\rho$}                            & \textbf{90.4\%} & 72.6\%             & 79.9\% & 81.9\% \\ \hline
\scalebox{0.75}[1]{GCC, $C_{ei}$, $\rho$ }& \textbf{90.3\%} & 59.2\%             & 76.3\% & 81.3\% \\ \hline
\end{tabular}

\label{tbl:ml_accuracy}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[h!]
% \centering
% \caption{\color{red}Top 10 accuracy score sorted by Random Forest for machine learning algorithms to classify 8 different generators by using triple of graph properties.}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% % Graph Properties                                 & Random Forest & Logistic Regression & SVM     & NN      \\ \hline
% % GCC, SCC,  $\rho$                        & 92.83\%       & 56.57\%             & 72.43\% & 88.08\% \\ \hline
% % GCC, SCC, APL                                    & 92.51\%       & 54.31\%             & 66.09\% & 62.39\% \\ \hline
% % GCC, SCC, den                                    & 92.48\%       & 56.74\%             & 72.44\% & 76.31\% \\ \hline
% % GCC, APL,  $\rho$                      & 92.03\%       & 55.18\%             & 70.59\% & 80.60\% \\ \hline
% % GCC, SCC, $\R_G$             & 91.91\%       & 57.42\%             & 75.67\% & 73.54\% \\ \hline
% % GCC, den, $\rho$                      & 91.73\%       & 54.14\%             & 91.24\% & 82.15\% \\ \hline
% % GCC, $\R_G$,  $\rho$ & 91.71\%       & 55.69\%             & 91.16\% & 77.78\% \\ \hline
% % GCC, edge   connectivity,  $\rho$        & 90.94\%       & 63.91\%             & 82.34\% & 81.99\% \\ \hline
% % GCC, den, $\R_G$            & 90.50\%       & 56.41\%             & 85.58\% & 75.48\% \\ \hline
% % GCC, r,  $\rho$                        & 90.36\%       & 72.64\%             & 79.86\% & 81.91\% \\ \hline
% Properties                                   & RF    & LR & SVM     & NN      \\ \hline
% GCC, SCC, $\rho$                         & \textbf{92.83\%} & 56.57\%             & 72.43\% & 88.08\% \\ \hline
% GCC, SCC, APL                                      & \textbf{92.51\%} & 54.31\%             & 66.09\% & 62.39\% \\ \hline
% GCC, SCC, den                                      & \textbf{92.48\%} & 56.74\%             & 72.44\% & 76.31\% \\ \hline
% GCC, APL, $\rho$                        & \textbf{92.03\%} & 55.18\%             & 70.59\% & 80.60\% \\ \hline
% GCC, SCC, $R_G$               & \textbf{91.91\%} & 57.42\%             & 75.67\% & 73.54\% \\ \hline
% GCC, den, $\rho$                       & \textbf{91.73\%} & 54.14\%             & 91.24\% & 82.15\% \\ \hline
% GCC, $C_e$, $\rho$            & \textbf{90.94\%} & 63.91\%             & 82.34\% & 81.99\% \\ \hline
% GCC, den, $R_G$             & \textbf{90.50\%} & 56.41\%             & 85.58\% & 75.48\% \\ \hline
% GCC, r, $\rho$                            & \textbf{90.36\%} & 72.64\%             & 79.86\% & 81.91\% \\ \hline
% GCC, $C_{ei}$, $\rho$ & \textbf{90.29\%} & 59.22\%             & 76.33\% & 81.31\% \\ \hline
% \end{tabular}
% \label{tbl:triples_ml_accuracy}
% \end{table}


==> Exploring the Space of Labeled Graphs/gd-graphs-stats.tex <==
\begin{table}[t]
\centering
\caption{
% The following properties tend to be on the the opposite ends of their ranges for graphs with small stress and small neighborhood preservation error. See for example the properties of the two graphs from
% Figure~\ref{fig:graph-drawings}.
In this table we illustrate the top ten differences between properties of the graphs in Figure~\ref{fig:graph-drawings}
% that differ the most, 
ordered by the property values.
}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% & $\rho$ & $R_G$ & den & diam & TW & VC & TD & $C_e$ & $C_C$ & $C_B$ & $\sigma $ & ASCC & $c_4$ & $r$ & GCC &  $C_{Eig}$& NP& APL \\ \hline
% value  &0.002&0.006&0.008&0.020&0.025&0.031&0.056&0.058&0.064&0.088&0.095&0.109&0.112&0.121&0.134&0.221&0.469&0.514 \\ \hline
% \end{tabular}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
& $C_C$ & $C_B$ & $\sigma $ & ASCC & $c_4$ & $r$ & GCC &  $C_{Eig}$& NP& APL \\ \hline
value  &0.064&0.088&0.095&0.109&0.112&0.121&0.134&0.221&0.469&0.514 \\ \hline
\end{tabular}

\label{Table:graph-drawings-props}
\end{table}


==> Exploring the Space of Labeled Graphs/known_bound_table.tex <==
\begin{table}[t]
\caption{Known bounds for some of the properties  \ErdosRenyi graphs. 
The first row shows the bounds for \ErdosRenyi graphs with $p = 1/2$ and the second row shows the bounds for \ErdosRenyi graphs with $p = \log (|V|) / |V|$. Note that the bounds of this table are for the non-normalized properties. Later, in Figure~\ref{fig:violin_conv_05} we show the normalized versions of these bounds.
}
\vspace{0.3cm}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
& GCC     & APL    & r     & den      & diam  & $R_G$    & $\rho$ \\ \hline
\scalebox{0.75}[1]{$p=1/2$}  & $p$~\cite{newman2018networks} &  \scalebox{0.75}[1]{$\frac{\ln(|V|)}{\ln(|V|-1)p}$}~\cite{newman2018networks} & $0$~\cite{newman2002assortative} & $p$ & 2~\cite{blass1979properties} &  \scalebox{0.5}[1]{$\leq|V|-1+\frac{2}{|V|-2}$}~\cite{ellens2011effective} & \scalebox{0.65}[1]{$(1+o(1)max(\sqrt{\Delta}, np)$}~\cite{krivelevich2003largest}\\ \hline

% APL_{norm} = \frac{ln(n)/(ln(n-1)p)}{(n+1)/6}

\scalebox{0.65}[1]{$p=\log(|V|)/|V|$} & $p$~\cite{newman2018networks}  & 
\scalebox{0.65}[1]{$\approx\frac{\ln(|V|)}{\ln(|V|-1)p}$}~\cite{newman2018networks} 
& 0~\cite{newman2002assortative} & $p$  &
\scalebox{0.65}[1]{$\approx \frac{\log(|V|)}{\log(|V|p)}$}~\cite{chung2001diameter}   
&{$\approx \frac{|V|}{p}$}~\cite{sylvester2016random} & \scalebox{0.65}[1]{$(1+o(1)max(\sqrt{\Delta}, np)$}~\cite{krivelevich2003largest} \\ \hline
\end{tabular}
% \vspace{.2cm}


\label{Table:converage_props}
\end{table}


==> Exploring the Space of Labeled Graphs/prediction_loss_table.tex <==
 % \begin{table}[t]
% \centering
%  \caption{Prediction results for the baseline mean estimator (the first row), the linear regression estimator (the second row) and the non-linear estimator, described in Section~\ref{sec:linear_analysis}. The columns correspond to $12$ graph properties.}

% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline

%  \scalebox{0.75}[1]{$L_1$ loss}       & \scalebox{0.75}[1]{GCC}     & \scalebox{0.75}[1]{ASCC}     & \scalebox{0.75}[1]{APL}     & \scalebox{0.75}[1]{r}       & \scalebox{0.75}[1]{den}     & \scalebox{0.75}[1]{diam}    & \scalebox{0.75}[1]{Ce}      
% %  & \scalebox{0.75}[1]{Cd}
%  & \scalebox{0.75}[1]{Cc}      & \scalebox{0.75}[1]{Cb}      & \scalebox{0.75}[1]{Cei}     & \scalebox{0.75}[1]{$R_G$}     & \scalebox{0.75}[1]{$\rho$}  \\ \hline
% \scalebox{0.75}[1]{mean}     & \scalebox{0.75}[1]{.00590} & \scalebox{0.75}[1]{.00092} & \scalebox{0.75}[1]{.00017} & \scalebox{0.75}[1]{.01129} & \scalebox{0.75}[1]{.00564} & \scalebox{0.75}[1]{0}    & \scalebox{0.75}[1]{.01735} 
% % & \scalebox{0.75}[1]{.01634}
% & \scalebox{0.75}[1]{.01723} & \scalebox{0.75}[1]{.00046} & \scalebox{0.75}[1]{.00488} & \scalebox{0.75}[1]{.00578} & \scalebox{0.75}[1]{.00562} \\ \hline
% \scalebox{0.75}[1]{linear}    & \scalebox{0.75}[1]{.00099} & \scalebox{0.75}[1]{.00003} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{.00771} & \scalebox{0.75}[1]{.00002} & \scalebox{0.75}[1]{0}    & \scalebox{0.75}[1]{.01046} 
% % & \scalebox{0.75}[1]{. 00033}
%  & \scalebox{0.75}[1]{.00035} & \scalebox{0.75}[1]{.00013} & \scalebox{0.75}[1]{.00075} & \scalebox{0.75}[1]{.00006} & \scalebox{0.75}[1]{.00004 }\\ \hline
% \scalebox{0.75}[1]{non-linear} &\scalebox{0.75}[1]{.00093} & \scalebox{0.75}[1]{.00002} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{.00241} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{0}    & \scalebox{0.75}[1]{.01004} 
% %& \scalebox{0.75}[1]{ .00000*}
% & \scalebox{0.75}[1]{.00000*}
% & \scalebox{0.75}[1]{.00011} & \scalebox{0.75}[1]{.00067} & \scalebox{0.75}[1]{.00004} & \scalebox{0.75}[1]{.00001} \\ \hline
% \end{tabular}
% \vspace{-.2cm}

% \label{table:prediction_feature_old}
% \end{table}

% \begin{table}[t]
% \centering
%  \caption{Prediction results for the baseline mean estimator (the first row), the linear regression estimator (the second row) and the non-linear estimator, described in Section~\ref{sec:linear_analysis}. The columns correspond to $13$ graph properties.}

% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline

%  \scalebox{0.75}[1]{$L_1$ loss}       & \scalebox{0.75}[1]{GCC}     & \scalebox{0.75}[1]{ASCC}     & \scalebox{0.75}[1]{APL}     & \scalebox{0.75}[1]{r}       & \scalebox{0.75}[1]{diam}     & \scalebox{0.75}[1]{den}    & \scalebox{0.75}[1]{Ce}     & \scalebox{0.75}[1]{Cc}      & \scalebox{0.75}[1]{Cb}      & \scalebox{0.75}[1]{Cei}    & \scalebox{0.75}[1]{$R_G$}     & \scalebox{0.75}[1]{$\rho$} & \scalebox{0.75}[1]{TW}  \\ \hline
 
% \scalebox{0.75}[1]{mean}     & \scalebox{0.75}[1]{.00606} & \scalebox{0.75}[1]{.00095} & \scalebox{0.75}[1]{.00017} & \scalebox{0.75}[1]{.01105} & \scalebox{0.75}[1]{.00000} & \scalebox{0.75}[1]{.00597}    & \scalebox{0.75}[1]{.01756} & \scalebox{0.75}[1]{.01832} & \scalebox{0.75}[1]{.00047} & \scalebox{0.75}[1]{.00523} & \scalebox{0.75}[1]{.00613} & \scalebox{0.75}[1]{.00592} & \scalebox{0.75}[1]{.00742} \\ \hline

% \scalebox{0.75}[1]{linear}    & \scalebox{0.75}[1]{.00096} & \scalebox{0.75}[1]{.00003} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{.00733} & \scalebox{0.75}[1]{.00000} & \scalebox{0.75}[1]{.00002}    & \scalebox{0.75}[1]{.01035} & \scalebox{0.75}[1]{.00193} & \scalebox{0.75}[1]{.00013} & \scalebox{0.75}[1]{.00075} & \scalebox{0.75}[1]{.00006} & \scalebox{0.75}[1]{.00003 } & \scalebox{0.75}[1]{.00652} \\ \hline
 
% \scalebox{0.75}[1]{non-linear} &\scalebox{0.75}[1]{.00092} & \scalebox{0.75}[1]{.00002} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{.00665} & \scalebox{0.75}[1]{.00000} & \scalebox{0.75}[1]{.00002}    & \scalebox{0.75}[1]{.01029} & \scalebox{0.75}[1]{.00183}
% & \scalebox{0.75}[1]{.00011} & \scalebox{0.75}[1]{.00067} & \scalebox{0.75}[1]{.00005} & \scalebox{0.75}[1]{.00002} & \scalebox{0.75}[1]{.00654} \\ \hline
% \end{tabular}
% \vspace{-.2cm}

% \label{table:prediction_feature_old}
% \end{table}



\begin{table}[t]
\centering
 \caption{Prediction results for the baseline mean estimator (the first row), the linear regression estimator (the second row) and the non-linear estimator, described in Section~\ref{sec:linear_analysis}. The columns correspond to $15$ graph properties.}

\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline

 \scalebox{0.75}[1]{$L_1$ loss}       & \scalebox{0.75}[1]{GCC}     & \scalebox{0.75}[1]{ASCC}     & \scalebox{0.75}[1]{APL}     & \scalebox{0.75}[1]{r}       & \scalebox{0.75}[1]{diam}     & \scalebox{0.75}[1]{den}    & \scalebox{0.75}[1]{Ce}     & \scalebox{0.75}[1]{Cc}      & \scalebox{0.75}[1]{Cb}      & \scalebox{0.75}[1]{Cei}    & \scalebox{0.75}[1]{$R_G$}     & \scalebox{0.75}[1]{$\rho$} & \scalebox{0.75}[1]{TW}  & \scalebox{0.75}[1]{TD} & \scalebox{0.75}[1]{VC} \\ \hline
 
\scalebox{0.75}[1]{mean}     & \scalebox{0.75}[1]{0.00575} & \scalebox{0.75}[1]{0.00091} & \scalebox{0.75}[1]{0.00017} & \scalebox{0.75}[1]{0.01128} & \scalebox{0.75}[1]{0.00000} & \scalebox{0.75}[1]{0.00558}    & \scalebox{0.75}[1]{0.01757} & \scalebox{0.75}[1]{0.01745} & \scalebox{0.75}[1]{0.00045} & \scalebox{0.75}[1]{0.00493} & \scalebox{0.75}[1]{0.00574} & \scalebox{0.75}[1]{0.00554} & \scalebox{0.75}[1]{0.00530} & \scalebox{0.75}[1]{0.00206} & \scalebox{0.75}[1]{0.00337} \\ \hline

\scalebox{0.75}[1]{linear}    & \scalebox{0.75}[1]{0.00093} & \scalebox{0.75}[1]{0.00003} & \scalebox{0.75}[1]{0.00000*} & \scalebox{0.75}[1]{0.00760} & \scalebox{0.75}[1]{0.00000} & \scalebox{0.75}[1]{0.00003}    & \scalebox{0.75}[1]{0.01033} & \scalebox{0.75}[1]{0.00198} & \scalebox{0.75}[1]{0.00013} & \scalebox{0.75}[1]{0.00076} & \scalebox{0.75}[1]{0.00006} & \scalebox{0.75}[1]{0.00004} & \scalebox{0.75}[1]{0.00377} & \scalebox{0.75}[1]{0.00283} & \scalebox{0.75}[1]{0.00306} \\ \hline
 
\scalebox{0.75}[1]{non-linear} &\scalebox{0.75}[1]{0.00092} & \scalebox{0.75}[1]{0.00002} & \scalebox{0.75}[1]{0.00000*} & \scalebox{0.75}[1]{0.00668} & \scalebox{0.75}[1]{0.00000} & \scalebox{0.75}[1]{0.00002} & \scalebox{0.75}[1]{0.01013} & \scalebox{0.75}[1]{0.00190} & \scalebox{0.75}[1]{0.00011} & \scalebox{0.75}[1]{0.00070} & \scalebox{0.75}[1]{0.00005} & \scalebox{0.75}[1]{0.00003} & \scalebox{0.75}[1]{0.00371} & 
\scalebox{0.75}[1]{0.00266} & \scalebox{0.75}[1]{0.00288} \\ \hline
\end{tabular}
\vspace{-.2cm}

\label{table:prediction_feature}
\end{table}





==> Exploring the Space of Labeled Graphs/prediction_loss_table_percent.tex <==
 % \begin{table}[t]
% \centering
%  \caption{Prediction results for the baseline mean estimator (the first row), the linear regression estimator (the second row) and the non-linear estimator, described in Section~\ref{sec:linear_analysis}. The columns correspond to $12$ graph properties.}

% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline

%  \scalebox{0.75}[1]{$L_1$ loss}       & \scalebox{0.75}[1]{GCC}     & \scalebox{0.75}[1]{ASCC}     & \scalebox{0.75}[1]{APL}     & \scalebox{0.75}[1]{r}       & \scalebox{0.75}[1]{den}     & \scalebox{0.75}[1]{diam}    & \scalebox{0.75}[1]{Ce}      
% %  & \scalebox{0.75}[1]{Cd}
%  & \scalebox{0.75}[1]{Cc}      & \scalebox{0.75}[1]{Cb}      & \scalebox{0.75}[1]{Cei}     & \scalebox{0.75}[1]{$R_G$}     & \scalebox{0.75}[1]{$\rho$}  \\ \hline
% \scalebox{0.75}[1]{mean}     & \scalebox{0.75}[1]{.00590} & \scalebox{0.75}[1]{.00092} & \scalebox{0.75}[1]{.00017} & \scalebox{0.75}[1]{.01129} & \scalebox{0.75}[1]{.00564} & \scalebox{0.75}[1]{0}    & \scalebox{0.75}[1]{.01735} 
% % & \scalebox{0.75}[1]{.01634}
% & \scalebox{0.75}[1]{.01723} & \scalebox{0.75}[1]{.00046} & \scalebox{0.75}[1]{.00488} & \scalebox{0.75}[1]{.00578} & \scalebox{0.75}[1]{.00562} \\ \hline
% \scalebox{0.75}[1]{linear}    & \scalebox{0.75}[1]{.00099} & \scalebox{0.75}[1]{.00003} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{.00771} & \scalebox{0.75}[1]{.00002} & \scalebox{0.75}[1]{0}    & \scalebox{0.75}[1]{.01046} 
% % & \scalebox{0.75}[1]{. 00033}
%  & \scalebox{0.75}[1]{.00035} & \scalebox{0.75}[1]{.00013} & \scalebox{0.75}[1]{.00075} & \scalebox{0.75}[1]{.00006} & \scalebox{0.75}[1]{.00004 }\\ \hline
% \scalebox{0.75}[1]{non-linear} &\scalebox{0.75}[1]{.00093} & \scalebox{0.75}[1]{.00002} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{.00241} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{0}    & \scalebox{0.75}[1]{.01004} 
% %& \scalebox{0.75}[1]{ .00000*}
% & \scalebox{0.75}[1]{.00000*}
% & \scalebox{0.75}[1]{.00011} & \scalebox{0.75}[1]{.00067} & \scalebox{0.75}[1]{.00004} & \scalebox{0.75}[1]{.00001} \\ \hline
% \end{tabular}
% \vspace{-.2cm}

% \label{table:prediction_feature_old}
% \end{table}

% \begin{table}[t]
% \centering
%  \caption{Prediction results for the baseline mean estimator (the first row), the linear regression estimator (the second row) and the non-linear estimator, described in Section~\ref{sec:linear_analysis}. The columns correspond to $13$ graph properties.}

% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline

%  \scalebox{0.75}[1]{$L_1$ loss}       & \scalebox{0.75}[1]{GCC}     & \scalebox{0.75}[1]{ASCC}     & \scalebox{0.75}[1]{APL}     & \scalebox{0.75}[1]{r}       & \scalebox{0.75}[1]{diam}     & \scalebox{0.75}[1]{den}    & \scalebox{0.75}[1]{Ce}     & \scalebox{0.75}[1]{Cc}      & \scalebox{0.75}[1]{Cb}      & \scalebox{0.75}[1]{Cei}    & \scalebox{0.75}[1]{$R_G$}     & \scalebox{0.75}[1]{$\rho$} & \scalebox{0.75}[1]{TW}  \\ \hline
 
% \scalebox{0.75}[1]{mean}     & \scalebox{0.75}[1]{.00606} & \scalebox{0.75}[1]{.00095} & \scalebox{0.75}[1]{.00017} & \scalebox{0.75}[1]{.01105} & \scalebox{0.75}[1]{.00000} & \scalebox{0.75}[1]{.00597}    & \scalebox{0.75}[1]{.01756} & \scalebox{0.75}[1]{.01832} & \scalebox{0.75}[1]{.00047} & \scalebox{0.75}[1]{.00523} & \scalebox{0.75}[1]{.00613} & \scalebox{0.75}[1]{.00592} & \scalebox{0.75}[1]{.00742} \\ \hline

% \scalebox{0.75}[1]{linear}    & \scalebox{0.75}[1]{.00096} & \scalebox{0.75}[1]{.00003} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{.00733} & \scalebox{0.75}[1]{.00000} & \scalebox{0.75}[1]{.00002}    & \scalebox{0.75}[1]{.01035} & \scalebox{0.75}[1]{.00193} & \scalebox{0.75}[1]{.00013} & \scalebox{0.75}[1]{.00075} & \scalebox{0.75}[1]{.00006} & \scalebox{0.75}[1]{.00003 } & \scalebox{0.75}[1]{.00652} \\ \hline
 
% \scalebox{0.75}[1]{non-linear} &\scalebox{0.75}[1]{.00092} & \scalebox{0.75}[1]{.00002} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{.00665} & \scalebox{0.75}[1]{.00000} & \scalebox{0.75}[1]{.00002}    & \scalebox{0.75}[1]{.01029} & \scalebox{0.75}[1]{.00183}
% & \scalebox{0.75}[1]{.00011} & \scalebox{0.75}[1]{.00067} & \scalebox{0.75}[1]{.00005} & \scalebox{0.75}[1]{.00002} & \scalebox{0.75}[1]{.00654} \\ \hline
% \end{tabular}
% \vspace{-.2cm}

% \label{table:prediction_feature_old}
% \end{table}



\begin{table}[t]
\centering
 \caption{Prediction error (in percentage) for the baseline mean estimator (the first row), the linear regression estimator (the second row) and the non-linear estimator, described in Section~\ref{sec:linear_analysis}. The columns correspond to the $15$ graph properties.}
\vspace{0.3cm}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline

 \scalebox{0.75}[1]{$L_1$ loss}       & \scalebox{0.75}[1]{GCC}     & \scalebox{0.75}[1]{ASCC}     & \scalebox{0.75}[1]{APL}     & \scalebox{0.75}[1]{r}       & \scalebox{0.75}[1]{diam}     & \scalebox{0.75}[1]{den}    & \scalebox{0.75}[1]{Ce}     & \scalebox{0.75}[1]{Cc}      & \scalebox{0.75}[1]{Cb}      & \scalebox{0.75}[1]{Cei}    & \scalebox{0.75}[1]{$R_G$}     & \scalebox{0.75}[1]{$\rho$} & \scalebox{0.75}[1]{TW}  & \scalebox{0.75}[1]{TD} & \scalebox{0.75}[1]{VC} \\ \hline
 
\scalebox{0.75}[1]{mean}     & \scalebox{0.75}[1]{0.575} & \scalebox{0.75}[1]{0.091} & \scalebox{0.75}[1]{0.017} & \scalebox{0.75}[1]{0.564} & \scalebox{0.75}[1]{0.000} & \scalebox{0.75}[1]{0.558}    & \scalebox{0.75}[1]{1.757} & \scalebox{0.75}[1]{1.745} & \scalebox{0.75}[1]{0.045} & \scalebox{0.75}[1]{0.493} & \scalebox{0.75}[1]{0.574} & \scalebox{0.75}[1]{0.554} & \scalebox{0.75}[1]{0.530} & \scalebox{0.75}[1]{0.206} & \scalebox{0.75}[1]{0.337} \\ \hline

\scalebox{0.75}[1]{linear}    & \scalebox{0.75}[1]{0.093} & \scalebox{0.75}[1]{0.003} & \scalebox{0.75}[1]{0.000*} & \scalebox{0.75}[1]{0.380} & \scalebox{0.75}[1]{0.000} & \scalebox{0.75}[1]{0.003}    & \scalebox{0.75}[1]{1.033} & \scalebox{0.75}[1]{0.198} & \scalebox{0.75}[1]{0.013} & \scalebox{0.75}[1]{0.076} & \scalebox{0.75}[1]{0.006} & \scalebox{0.75}[1]{0.004} & \scalebox{0.75}[1]{0.377} & \scalebox{0.75}[1]{0.283} & \scalebox{0.75}[1]{0.306} \\ \hline
 
\scalebox{0.75}[1]{non-linear} &\scalebox{0.75}[1]{0.092} & \scalebox{0.75}[1]{0.002} & \scalebox{0.75}[1]{0.000*} & \scalebox{0.75}[1]{0.334} & \scalebox{0.75}[1]{0.000} & \scalebox{0.75}[1]{0.002} & \scalebox{0.75}[1]{1.013} & \scalebox{0.75}[1]{0.190} & \scalebox{0.75}[1]{0.011} & \scalebox{0.75}[1]{0.070} & \scalebox{0.75}[1]{0.005} & \scalebox{0.75}[1]{0.003} & \scalebox{0.75}[1]{0.371} & 
\scalebox{0.75}[1]{0.266} & \scalebox{0.75}[1]{0.288} \\ \hline
\end{tabular}
\vspace{-.2cm}

\label{table:prediction_feature}
\end{table}





==> Exploring the Space of Labeled Graphs/properties_example.tex <==
\begin{figure*}[ht]
\centering
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/4486_high_apl}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/146036_mid_apl}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/261053_low_apl}
\caption{APL is the average of the shortest paths of all pairs. As the graph in left graph has almost a path structure, degree of the vertices are very low, therefore, they are connected to few vertices. That makes the shortest paths greater(APL=0.95). So, APL value is greater for left graph. The graph in middle one has more edges, making the shortest paths a little smaller(APL=0.66). right graph has the most edges making the vertices better connected. Almost each vertex have a path of length \(1\) to another vertex. So, APL is lower than other two(APL=0.325). }
  \label{fig:apl_examples}
\end{figure*}

\begin{figure*}[ht]
\centering
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/260766_high_den}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/219525_mid_den}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/23772_low_den}
    \caption{Density is calculated by the proportion of number of present edges and  possible edges. As left graph has the highest number of edges in this figure, density value of left one is also the highest(den=0.92). The middle graph have less edges compare to left one(den=0.69). The right graph have only 10 edges(den=0.28)}
  \label{fig:den_examples}
\end{figure*}

\begin{figure*}[ht]
\centering
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/64550_high_diam}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/23020_mid_diam}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/261079_low_diam}
\caption{We are showing the normalized diameter here. Diameter is the longest shortest paths of the vertex-pairs. left graph has the longest shortest path \(7\)(diam=0.875, after normalized). The middle graph has the longest shortest path \(4\)(diam=0.5) while right graph has longest shortest path \(1\)(diam=0.125).}
  \label{fig:diam_examples}
\end{figure*}

\begin{figure*}[ht]
    \includegraphics[width=0.3\textwidth]{./figures/prop_examples/high_r}
    \includegraphics[width=0.2\textwidth,angle=90]{./figures/prop_examples/medium_r}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/29_high_r}
    \caption{The left graph have $r=0.81$, middle one have $r=0$ and the right one have $r=0.98$ In left graph, most of the vertices are connected to vertices with similar degree values. The right graph is opposite. The low-degree vertices are connected to high-degree vertices. Therefore, these two have these two extreme values. On the other hand, the one in the middle does not create any community of high-degree and low-degree vertices. All of the vertices have very close degree value. So, degree assortativity is \(0\). }
  \label{fig:r_examples}
\end{figure*}

\begin{figure*}[ht]
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/261077_high_ce}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/256444_mid_ce}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/256537_low_ce}
    \caption{The left graph have $C_E = 0.87$, middle one have$C_E = 0.62$ and right one have $C_E = 0.12$. as shown in graph, with higher $C_E$, the graph are more connected and hard to disconnected. In the right graph, we can easily  disconnected the graph by removing only one edge. Therefore, edge connectivity is small.}
  \label{fig:ce_examples}
\end{figure*}

\begin{figure*}[ht]
\includegraphics[width=0.3\textwidth]{./figures/prop_examples/7_high_degree}
\includegraphics[width=0.3\textwidth]{./figures/prop_examples/mid_degree.pdf}
\includegraphics[width=0.3\textwidth]{./figures/prop_examples/low_degree1.pdf}
\caption{$C_D$ for left, middle and right graphs is $0.93, 0.5, 0.13$, respectively. left and middle graphs both has one high-degree vertices. the high-degree vertices in left graph is connected to all of the vertices and all other vertices have only small degrees. The middle graph have several vertices that have degree more than $4$, Therefore the  $C_D$ for it is not as high as left one.  vertices in the right graph almost have  similar degrees. So, $C_D$ is small.}
  \label{fig:dc_examples}
\end{figure*}

\begin{figure*}[ht]
    \includegraphics[width=0.3\textwidth,angle=90]{./figures/prop_examples/37_high_cc}
    \includegraphics[width=0.3\textwidth,angle=90]{./figures/prop_examples/257115_mid_cc}
    \includegraphics[width=0.3\textwidth,angle=90]{./figures/prop_examples/248698_low_cc}
    \caption{$C_c$ for left, middle and right graphs is $0.96, 0.47, ~0$, respectively. left and middle graphs both have high-degree vertices. the only high-degree vertices in left graph is connected to most of the vertices and all other vertices have only small degrees. Most vertices in middle graph have high degree. Therefore the correlation for it is not as high as left one. vertices in the right graph are far from each other.}
  \label{fig:cc_examples}
\end{figure*}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[ht]
    \includegraphics[width=0.3\textwidth,angle=90]{./figures/prop_examples/2_high_between}
    \includegraphics[width=0.3\textwidth,angle=90]{./figures/prop_examples/256550_mid_between}
\includegraphics[width=0.3\textwidth]{./figures/prop_examples/low_between}
  \caption{$C_B$ for left, middle and right graphs is $0.96, 0.52, 0.06$, respectively. }
  \label{fig:bet_examples}
\end{figure*}

\begin{figure*}[ht]
    \includegraphics[width=0.31\textwidth,angle=90]{./figures/prop_examples/35_high_eigen}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/4551_mid_eigen}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/256483_low_eigen}
    \caption{$C_{ei}$ for left, middle and right graphs is $0.95, 0.49, ~0$, respectively.}
  \label{fig:cei_examples}
\end{figure*}

% \begin{figure*}[h]
% \centering
% \begin{subfigure}{\dis\textwidth}
%     \centering
%     \includegraphics[width=0.7\textwidth,angle=90]{./figures/prop_examples/261078_high_egr}
%     \caption{A graph with $|V|=9, |E|=35, E\_G\_resist=0.965517241 $ }
%     \label{fig:high_egr}
% \end{subfigure}
% \begin{subfigure}{\dis\textwidth}
%     \centering
%     \includegraphics[width=0.7\textwidth,angle=90]{./figures/prop_examples/195985_mid_egr}
%     \caption{A graph with $|V|=9, |E|=26, E\_G\_resist=0.630631 $ }
%     \label{fig:mid_egr}
% \end{subfigure}
% \begin{subfigure}{\dis\textwidth}
%     \centering
%     \includegraphics[width=0.7\textwidth,angle=90]{./figures/prop_examples/146067_low_egr}
%     \caption{A graph with $|V|=9, |E|=16, E\_G\_resist=0.263158 $ }
%     \label{fig:low_egr}
%     \end{subfigure}
%     \caption{Graphs with high, medium and low-valued effective graph resistance.}
%   \label{fig:egr_examples}
% \end{figure*}

% \begin{figure*}[h]
% \centering
% \begin{subfigure}{\dis\textwidth}
%     \centering
%     \includegraphics[width=0.7\textwidth,angle=90]{./figures/prop_examples/261054_high_sr}
%     \caption{A graph with $|V|=9, |E|=34, S_{rad}=0.950694 $ }
%     \label{fig:high_sr}
% \end{subfigure}
% \begin{subfigure}{\dis\textwidth}
%     \centering
%     \includegraphics[width=0.7\textwidth,angle=90]{./figures/prop_examples/22649_mid_sr}
%     \caption{A graph with $|V|=9, |E|=15, S_{rad}=0.503142969 $ }
%     \label{fig:mid_sr}
% \end{subfigure}
% \begin{subfigure}{\dis\textwidth}
%     \centering
%     \includegraphics[width=0.7\textwidth,angle=90]{./figures/prop_examples/24344_low_sr}
%     \caption{A graph with $|V|=9, |E|=8, S_{rad}=0.237764 $ }
%     \label{fig:low_sr}
%     \end{subfigure}
%     \caption{Graphs with high, medium and low-valued spectral radius. Spectral radius shows us the relation of average degree and the highest degree in the graph. For any graph with specific number of vertices, the range of spectral radius is from average degree to the highest degree in that graph. The first graph here has an average of around 7.5 degree which will be around 0.94 if normalized. The highest degree in this graph is 8, i.e; 1 as normalized. The graph is (b), however has a lower average, 0.42 as normalized. The last graph has 0.22 as average and 0.25 as highest degree. We can see that all of the spectral radius is in this range. }
%     % https://www.epfl.ch/labs/dcg/wp-content/uploads/2018/10/ADM-Eigenvalues-v3.pdf
%   \label{fig:sr_examples}
% \end{figure*}


==> Exploring the Space of Labeled Graphs/properties_trends_ER_0.5.tex <==

\begin{figure}[htp!]
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_GCC}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_SCC}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_APL}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_r}
	
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_diam}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_den}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Ce}
% 	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Cd}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Cc}
	
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Cb}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_Cei}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_R_G_new}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_s_rad}
    
    % \includegraphics[width=.24\textwidth]{./figures/trends/ER_TW_apr}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_TW}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_TD}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_VC}
    
    % \includegraphics[width=.98\textwidth, height=0.003\textwidth]{figures/balck_line}
  
\caption{Behavior of graph properties for $1000$ graphs generated according to \ErdosRenyi model with $p = 1/2$. The number of vertices is in the range $[5,10,..,100]$ and the results are illustrated with violin plots. The first row shows the results for GCC, ASCC, APL and $r$.
The second row includes diameter, density, $C_e$ and $C_C$. The third row includes $C_V$, $C_{Eig}$, $R_G$ and $\rho$. The fourth row includes TW, TD, and VC.
}
	\label{fig:violin_conv_05}
	\centering
\end{figure}

\begin{comment}
\begin{figure}[ht!]
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_GCC}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_SCC}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_APL}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_r}
	
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_diam}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_den}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Ce}
% 	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Cd}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Cc}
	
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Cb}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_Cei}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_R_G_new}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_s_rad}
    
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_TW}
    
    \includegraphics[width=.98\textwidth, height=0.003\textwidth]{figures/balck_line}
    
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_GCC}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_SCC}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_APL}
    \includegraphics[width=.24\textwidth]{./figures/trends/ERlog_r}
    
    \includegraphics[width=.24\textwidth]{./figures/trends/ERlog_diam}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_den}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Ce}
% 	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Cd}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Cc}
	
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Cb}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Cei}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_R_G}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_s_rad}
	
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_TW}

\caption{Behavior of graph properties for $1000$ graphs generated according to \ErdosRenyi model. The first three rows include the results for \ErdosRenyi with $p = 1/2$ and the bottom three rows include the results for the \ErdosRenyi model with $p=\log|V|/|V|$. The number of vertices is in the range $[5,10,..,100]$ and the results are illustrated with violin plots. The first row shows the results for Global Clustering Coefficient, Average Square Clustering, Average Path Length and Degree Assortativity.
The second row includes Diameter, Density, Edge Connectivity and Closeness Centrality. The third row includes Betweenness Centrality, Eigenvector Centrality, Effective Graph Resistance and Spectral Radius. The fourth, fifth and sixth rows show the same data for $p=\log|V|/|V|$.
}
	\label{fig:violin_conv}
	\centering
\end{figure}

\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\begin{figure}[h!]
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_GCC}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_SCC}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_APL}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_r}
	
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_diam}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_den}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Ce}
% 	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Cd}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Cc}
	
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Cb}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_Cei}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_R_G_new}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_s_rad}
	
	\caption{Behaviour of graph properties for $1000$ graphs generated according to \ErdosRenyi model with $p = 1/2$ and values of $|V|$ in the range $[5,10,..,100]$.  The results are illustrated with violin plots. The first row shows the results for Global Clustering Coefficient, Average Square Clustering, Average Path Length and Degree Assortativity. 
	The second row shows Diameter, Density, Edge Connectivity and Closeness Centrality. The third row shows Betweenness Centrality, Eigenvector Centrality, Effective Graph Resistance and Spectral Radius.
% 	The second row shows Diameter, Density, Edge Connectivity and Degree Centrality. The third row shows Closeness Centrality, Betweenness Centrality, Eigenvector Centrality and Effective Graph Resistance. The last row shows Spectral Radius.
	}
	\label{fig:violin_conv_1}
	\centering
\end{figure}

\begin{figure}[h]
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_GCC}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_SCC}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_APL}
    \includegraphics[width=.24\textwidth]{./figures/trends/ERlog_r}
    
    \includegraphics[width=.24\textwidth]{./figures/trends/ERlog_diam}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_den}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Ce}
% 	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Cd}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Cc}
	
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Cb}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Cei}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_R_G}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_s_rad}


	\caption{Behaviour of graph properties for $1000$ graphs generated according to \ErdosRenyi model with $p = \log|V|/|V|$
 and values of $|V|$ in the range $[5,10,..,100]$.  The results are illustrated with violin plots. The first row shows the results for Global Clustering Coefficient, Average Square Clustering, Average Path Length and Degree Assortativity.
  The second row shows Diameter, Density, Edge Connectivity and Closeness Centrality. The third row shows Betweenness Centrality, Eigenvector Centrality, Effective Graph Resistance and Spectral Radius.
%  The second row shows Diameter, Density, Edge Connectivity and Degree Centrality. The third row shows Closeness Centrality, Betweenness Centrality, Eigenvector Centrality and Effective Graph Resistance. The last row shows Spectral Radius.
 }
	\label{fig:violin_conv_2}
	\centering
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[ht]
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_GCC}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_SCC}
    \includegraphics[width=.24\textwidth]{./figures/trends/ER_APL}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_r}
	
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_GCC}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_SCC}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_APL}
    \includegraphics[width=.24\textwidth]{./figures/trends/ERlog_r}
	\caption{Demonstration of the behaviour of graph properties for graphs generated by the \ErdosRenyi model. The top row contains results for \ErdosRenyi model with $p = 1/2$ and the bottom row contains the results for \ErdosRenyi model with $p=log(|V|)/|V|$. Each column presents results for one property from left to right the properties are: Global Clustering Coefficient, Average Square Clustering, Average Path Length and Degree Assortativity. For each experiment we generated 1,000 graphs according to \ErdosRenyi model for $p = 1/2$ for the top row and $p=log(|V|)/|V|$ for the bottom row varying $|V| = 5,10,..,80$. The results are demonstrated as violin plots.}
	\label{fig:violin_conv_1}
	\centering
\end{figure}

\begin{figure}[ht]
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_diam}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_den}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Ce}
	\includegraphics[width=.24\textwidth]{./figures/trends/ER_Cd}

	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_diam}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_den}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Ce}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Cd}

	\caption{Demonstration of the behaviour of graph properties for graphs generated by the \ErdosRenyi model. The top row contains results for \ErdosRenyi model with $p = 1/2$ and the bottom row contains the results for \ErdosRenyi model with $p=log(|V|)/|V|$. Each column presents results for one property from left to right the properties are: Diameter, Density, Edge Connectivity and Degree Centrality. For each experiment we generated 1,000 graphs according to \ErdosRenyi model for $p = 1/2$ for the top row and $p=log(|V|)/|V|$ for the bottom row varying $|V| = 5,10,..,80$. The results are demonstrated as violin plots.}
	\label{fig:violin_conv_2}
	\centering
\end{figure}

\begin{figure}[ht]
	\includegraphics[width=.195\textwidth]{./figures/trends/ER_Cc}
	\includegraphics[width=.195\textwidth]{./figures/trends/ER_Cb}
    \includegraphics[width=.195\textwidth]{./figures/trends/ER_Cei}
    \includegraphics[width=.195\textwidth]{./figures/trends/ER_R_G}
    \includegraphics[width=.195\textwidth]{./figures/trends/ER_s_rad}

	\includegraphics[width=.195\textwidth]{./figures/trends/ERlog_Cc}
	\includegraphics[width=.195\textwidth]{./figures/trends/ERlog_Cb}
	\includegraphics[width=.195\textwidth]{./figures/trends/ERlog_Cei}
	\includegraphics[width=.195\textwidth]{./figures/trends/ERlog_R_G}
	\includegraphics[width=.195\textwidth]{./figures/trends/ERlog_s_rad}

	\caption{Demonstration of the behaviour of graph properties for graphs generated by the \ErdosRenyi model. The top row contains results for \ErdosRenyi model with $p = 1/2$ and the bottom row contains the results for \ErdosRenyi model with $p=log(|V|)/|V|$. Each column presents results for one property from left to right the properties are: Closeness Centrality, Betweenness Centrality, Eigenvector Centrality, Effective Graph Resistance, Spectral Radius. For each experiment we generated 1,000 graphs according to \ErdosRenyi model for $p = 1/2$ for the top row and $p=log(|V|)/|V|$ for the bottom row varying $|V| = 5,10,..,80$. The results are demonstrated as violin plots.}
	\label{fig:violin_conv_3}
	\centering
\end{figure}

\end{comment}

\begin{comment}
\begin{figure}[ht]
	\includegraphics[width=.5\textwidth]{./figures/trends/ER_GCC}
	\includegraphics[width=.5\textwidth]{./figures/trends/ERlog_GCC}
	\caption{the left and right plot respected to ER model with $p=1/2$ and $p=log(|V|)/|V|$. We generated 1,000 graphs for different $p$ and for each $|V| = 5,10,..,80$. Thus, each plot is a series of violin plots for one properties that vary $|V|$ from 5 to 80.}
	\label{fig:violin_GCC}
	\centering
\end{figure}
\begin{figure}[ht]
	\includegraphics[width=.5\textwidth]{./figures/trends/ER_SCC}
	\includegraphics[width=.5\textwidth]{./figures/trends/ERlog_SCC}
	\caption{the left and right plot respected to ER model with $p=1/2$ and $p=log(|V|)/|V|$. We generated 1,000 graphs for different $p$ and for each $|V| = 5,10,..,80$. Thus, each plot is a series of violin plots for one properties that vary $|V|$ from 5 to 80.}
	\label{fig:violin_SCC}
	\centering
\end{figure}
\begin{figure}[ht]
	\includegraphics[width=.5\textwidth]{./figures/trends/ER_APL}
	\includegraphics[width=.5\textwidth]{./figures/trends/ERlog_APL}
	\caption{the left and right plot respected to ER model with $p=1/2$ and $p=log(|V|)/|V|$. We generated 1,000 graphs for different $p$ and for each $|V| = 5,10,..,80$. Thus, each plot is a series of violin plots for one properties that vary $|V|$ from 5 to 80.}
	\label{fig:violin_APL}
	\centering
\end{figure}
\begin{figure}[ht]
	\includegraphics[width=.5\textwidth]{./figures/trends/ER_r}
	\includegraphics[width=.5\textwidth]{./figures/trends/ERlog_r}
	\caption{the left and right plot respected to ER model with $p=1/2$ and $p=log(|V|)/|V|$. We generated 1,000 graphs for different $p$ and for each $|V| = 5,10,..,80$. Thus, each plot is a series of violin plots for one properties that vary $|V|$ from 5 to 80.}
	\label{fig:violin_r}
	\centering
\end{figure}
\begin{figure}[ht]
	\includegraphics[width=.5\textwidth]{./figures/trends/ER_diam}
	\includegraphics[width=.5\textwidth]{./figures/trends/ERlog_diam}
	\caption{the left and right plot respected to ER model with $p=1/2$ and $p=log(|V|)/|V|$. We generated 1,000 graphs for different $p$ and for each $|V| = 5,10,..,80$. Thus, each plot is a series of violin plots for one properties that vary $|V|$ from 5 to 80.}
	\label{fig:violin_diam}
	\centering
\end{figure}
\begin{figure}[ht]
	\includegraphics[width=.5\textwidth]{./figures/trends/ER_den}
	\includegraphics[width=.5\textwidth]{./figures/trends/ERlog_den}
	\caption{the left and right plot respected to ER model with $p=1/2$ and $p=log(|V|)/|V|$. We generated 1,000 graphs for different $p$ and for each $|V| = 5,10,..,80$. Thus, each plot is a series of violin plots for one properties that vary $|V|$ from 5 to 80.}
	\label{fig:violin_den}
	\centering
\end{figure}
\begin{figure}[ht]
	\includegraphics[width=.5\textwidth]{./figures/trends/ER_Ce}
	\includegraphics[width=.5\textwidth]{./figures/trends/ERlog_Ce}
	\caption{the left and right plot respected to ER model with $p=1/2$ and $p=log(|V|)/|V|$. We generated 1,000 graphs for different $p$ and for each $|V| = 5,10,..,80$. Thus, each plot is a series of violin plots for one properties that vary $|V|$ from 5 to 80.}
	\label{fig:violin_Ce}
	\centering
\end{figure}
\begin{figure}[ht]
	\includegraphics[width=.5\textwidth]{./figures/trends/ER_Cd}
	\includegraphics[width=.5\textwidth]{./figures/trends/ERlog_Cd}
	\caption{the left and right plot respected to ER model with $p=1/2$ and $p=log(|V|)/|V|$. We generated 1,000 graphs for different $p$ and for each $|V| = 5,10,..,80$. Thus, each plot is a series of violin plots for one properties that vary $|V|$ from 5 to 80.}
	\label{fig:violin_Cd}
	\centering
\end{figure}
\begin{figure}[ht]
	\includegraphics[width=.5\textwidth]{./figures/trends/ER_Cc}
	\includegraphics[width=.5\textwidth]{./figures/trends/ERlog_Cc}
	\caption{the left and right plot respected to ER model with $p=1/2$ and $p=log(|V|)/|V|$. We generated 1,000 graphs for different $p$ and for each $|V| = 5,10,..,80$. Thus, each plot is a series of violin plots for one properties that vary $|V|$ from 5 to 80.}
	\label{fig:violin_Cc}
	\centering
\end{figure}
\begin{figure}[ht]
	\includegraphics[width=.5\textwidth]{./figures/trends/ER_Cb}
	\includegraphics[width=.5\textwidth]{./figures/trends/ERlog_Cb}
	\caption{the left and right plot respected to ER model with $p=1/2$ and $p=log(|V|)/|V|$. We generated 1,000 graphs for different $p$ and for each $|V| = 5,10,..,80$. Thus, each plot is a series of violin plots for one properties that vary $|V|$ from 5 to 80.}
	\label{fig:violin_Cb}
	\centering
\end{figure}
\begin{figure}[ht]
	\includegraphics[width=.5\textwidth]{./figures/trends/ER_Cei}
	\includegraphics[width=.5\textwidth]{./figures/trends/ERlog_Cei}
	\caption{the left and right plot respected to ER model with $p=1/2$ and $p=log(|V|)/|V|$. We generated 1,000 graphs for different $p$ and for each $|V| = 5,10,..,80$. Thus, each plot is a series of violin plots for one properties that vary $|V|$ from 5 to 80.}
	\label{fig:violin_Cei}
	\centering
\end{figure}
\begin{figure}[ht]
	\includegraphics[width=.5\textwidth]{./figures/trends/ER_R_G}
	\includegraphics[width=.5\textwidth]{./figures/trends/ERlog_R_G}
	\caption{the left and right plot respected to ER model with $p=1/2$ and $p=log(|V|)/|V|$. We generated 1,000 graphs for different $p$ and for each $|V| = 5,10,..,80$. Thus, each plot is a series of violin plots for one properties that vary $|V|$ from 5 to 80.}
	\label{fig:violin_resist}
	\centering
\end{figure}
\begin{figure}[ht]
	\includegraphics[width=.5\textwidth]{./figures/trends/ER_s_rad}
	\includegraphics[width=.5\textwidth]{./figures/trends/ERlog_s_rad}
	\caption{the left and right plot respected to ER model with $p=1/2$ and $p=log(|V|)/|V|$. We generated 1,000 graphs for different $p$ and for each $|V| = 5,10,..,80$. Thus, each plot is a series of violin plots for one properties that vary $|V|$ from 5 to 80.}
	\label{fig:violin_rad}
	\centering
\end{figure}

\end{comment}


==> Exploring the Space of Labeled Graphs/properties_trends_ER_log.tex <==

\begin{figure}[htp!]
	
    % \includegraphics[width=.98\textwidth, height=0.003\textwidth]{figures/balck_line}
    
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_GCC}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_SCC}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_APL}
    \includegraphics[width=.24\textwidth]{./figures/trends/ERlog_r}
    
    \includegraphics[width=.24\textwidth]{./figures/trends/ERlog_diam}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_den}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Ce}
% 	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Cd}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Cc}
	
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Cb}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_Cei}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_R_G}
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_s_rad}
	
	\includegraphics[width=.24\textwidth]{./figures/trends/ERlog_TW}

\caption{Behavior of graph properties for $1000$ graphs generated according to \ErdosRenyi model with $p = \log(|V|) / |V|$. The number of vertices is in the range $[5,10,..,100]$ and the results are illustrated with violin plots. The first row shows the results for Global Clustering Coefficient, Average Square Clustering, Average Path Length and Degree Assortativity.
The second row includes Diameter, Density, Edge Connectivity and Closeness Centrality. The third row includes Betweenness Centrality, Eigenvector Centrality, Effective Graph Resistance and Spectral Radius. The fourth row includes the results for Treewidth, TreeDepth and Vertex Covering.
}
	\label{fig:violin_conv_log}
	\centering
\end{figure}


==> Exploring the Space of Labeled Graphs/propertytable.tex <==

\begin{table}[t]

\caption{The set of graph properties considered in this paper. The first column includes the name of the property. The second column shows the formula (or the name of a solver) by which these properties can be computed for given graphs. The third column presents the time complexity of calculating the property and the last column includes relevant references.} % title of Table
\vspace{0.3cm}
\label{table:properties}
%\centering % used for centering table
%\rowcolors{2}{gray!25}{white}
{
\renewcommand{\arraystretch}{1.5}%
% \begin{tabular}
\begin{tabular}{ m{3.2cm} m{6cm} m{1.4cm} m{1.2cm} } % centered columns (4 columns)
    %\rowcolor{gray!50}

\hline\hline %inserts double horizontal lines
  Name & Formula & time & Reference\\ % inserts table
%heading
\hline % inserts single horizontal line

\scalebox{0.75}[1]{Global Clustering Coeff.} %\\(transitivity)
& $GCC(G) =\frac{ 3 \times |\text{triangles}|}{|\text{connected triples in the graph}|}$& \scalebox{0.65}[1]{$O(|V|^3)$}&~\cite{chakrabarti2006graph,kairam2012graphprism}  \\

\scalebox{0.75}[1]{Average Sq. Clustering Coeff.}& \scalebox{0.85}[1]{$ASCC(G) =  \frac{1}{n} \sum_{i=1}^n c_4(u_i), u_i \in V,  n = |V| $} &\scalebox{0.65}[1]{$O(|V|^4)$}& \multirow{2}{*} ~\cite{lind2005cycles} \\  & $c_4(u_i) = \frac{\sum_{u=1}^{k_v}\sum_{w=u+1}^{k_v}q_v(u,w)}{\sum_{u=1}^{k_v}\sum_{w=u+1}^{k_v}[a_v(u,w)+q_v(u,w)] }$&\\

\scalebox{0.75}[1]{Average Path Length}& $APL(G) = \frac{1}{n(n-1)}\sum_{u,v \in V}d(u,v)$&\scalebox{0.65}[1]{$O(|V|^3)$}&~\cite{chakrabarti2007graph,li2011graph,chakrabarti2006graph,mislove2007measurement}\\

\scalebox{0.75}[1]{Degree Assortativity}& $r(G) = \frac{\sum_{xy}xy(e_{xy}-a_xb_y) }{\sigma_a \sigma_b}$&\scalebox{0.65}[1]{$O(|V|+|E|)$}&~\cite{newman2003mixing,mislove2007measurement}\\

\scalebox{0.75}[1]{Density} & $\den = \frac{2|E|}{|V|(|V| - 1)}$ & \scalebox{0.65}[1]{$O(1)$}&\\

\scalebox{0.75}[1]{Diameter}& $\diam(G) = \max\{\dist(v,w), v,w \in V \}$ &\scalebox{0.65}[1]{$O(|V||E|)$}& ~\cite{chakrabarti2007graph,mcglohon2011statistical,kairam2012graphprism,mislove2007measurement}\\

\scalebox{0.75}[1]{Edge Connectivity} & Ce: the minimum number of edges \shortstack{\\ to remove to disconnect the graph} &\scalebox{0.65}[1]{$O(|V||E|)$}& ~\cite{even1975network}\\

% \scalebox{0.75}[1]{Degree Centrality}&$C_D(v) = degree(v)  $ &\scalebox{0.65}[1]{$O(1)$}& ~\cite{lohmann2010eigenvector,newman2018networks}\\


\scalebox{0.75}[1]{Closeness Centrality} & $C_C(G)$; see~\eqref{eq:freeman_cent}. $C_C(G, v) = \frac{n-1}{\sum_{u\neq v}d(u,v)}  $ &\scalebox{0.65}[1]{$O(|V||E|)$}& ~\cite{wasserman1994social,newman2018networks}\\

\scalebox{0.75}[1]{Betweenness Centrality}& $C_B(G)$; see~\eqref{eq:freeman_cent}. $C_B(G, v) =\sum_{s,t \in V} \frac{\sigma(s,t|v)}{\sigma(s,t)}$ &\scalebox{0.65}[1]{$O(|V|^2 \log(|V|))$}
& ~\cite{barthelemy2004betweenness,brandes2001faster,brandes2008variants,leydesdorff2007betweenness,newman2018networks}\\
%  https://onlinelibrary.wiley.com/doi/full/10.1002/asi.20614
\scalebox{0.75}[1]{Eigenvector Centrality }&$C_{Eig}(G)$; see~\eqref{eq:freeman_cent}. $A$ is the adjacency matrix and $C_{Eig}(G, v) = \sum_{u\in V} A_{v,u} C_{Eig}(G, u)$  &\scalebox{0.65}[1]{$O(|V|^3)$}& ~\cite{bonacich1987power,costenbader2003stability,borgatti2005centrality,lohmann2010eigenvector,newman2018networks}\\
% The stability of centrality measures when networks are sampled:https://www.sciencedirect.com/science/article/pii/S0378873303000121
% https://www.sciencedirect.com/science/article/pii/S0378873304000693


% \scalebox{0.75}[1]{\sout{Freeman's Centralization}} &\scalebox{0.8}[1]{$C_x(G) = \frac{\sum_{v\in V}(C_x(n^*)-C_x(v))}{max\sum_{v\in V}(C_x(n^*)-C_x(v))}$, $x \in \{D,B,C,E\}$} &\scalebox{0.65}[1]{$O(|V|C_x)$}
% the denominator is the graph that have largest C_x in Ground Truth with same $|V|$
% & ~\sout{\cite{freeman1978centrality}}\\


\scalebox{0.75}[1]{Effective Graph Resistance}&$R_G = |V|\sum_{k=1}^{|V|-1}\frac{1}{\mu_k}$, 
% $\mu_k$ is the kth largest eigenvalue of its Laplacian matrix 
&\scalebox{0.65}[1]{$O(|V|^3)$}
&~\cite{li2011graph,ellens2011effective}\\

\scalebox{0.75}[1]{Spectral Radius}&$\rho(G) = |\lambda_1|$
%, the largest eigenvalue of its adjacency matrix
&\scalebox{0.65}[1]{$O(|V|^3)$}
&~\cite{li2011graph,berman2001spectral,friedland1988bounds}\\

\scalebox{0.75}[1]{Treewidth}
& \textsc{tidlib}; see Sec.~\ref{sec:def_properties}
&NP-Hard
&~\cite{bodlaender2005discovering,bodlaender2010treewidth,pace-tw}\\

\scalebox{0.75}[1]{Treedepth}
& \textsc{Bute-plus}; see Sec.~\ref{sec:def_properties}
&NP-Hard
&~\cite{pace-td}\\

\scalebox{0.75}[1]{Vertex cover}
& \textsc{WeGotYouCovered}; see Sec.~\ref{sec:def_properties}
&NP-Hard
&~\cite{pace-vc}\\

 %\\ [1ex] adds vertical space
\hline %inserts single line
\end{tabular}}
\end{table}


==> Exploring the Space of Labeled Graphs/same_stat.tex <==
\begin{figure}[t]
	\includegraphics[width=.24\textwidth]{./figures/same_stat/same_stat_v=100_1}
	\includegraphics[width=.24\textwidth]{./figures/same_stat/same_stat_v=100_2}
	\includegraphics[width=.24\textwidth]{./figures/same_stat/same_stat_v=100_3}
	\includegraphics[width=.24\textwidth]{./figures/same_stat/same_stat_v=100_4}

	\caption{ Four graphs generated by the \ErdosRenyi model with $p=1/2$ and $|V|=100$, with the same 12 properties (up to 2 decimal places). In $1000$  generated graphs, on average there are 78 pairs, 15 triples and 3 quadruples with the same 12 properties. Note that the graphs are not isomorphic to each other.}
	%since they have different degree sequences.}
	\label{fig:same_stat_4_tuple}
	\centering
\end{figure}
% \todo{remove this figure?}

==> gd-graphs-stats.tex <==
\begin{table}[t]
\centering
\caption{
% The following properties tend to be on the the opposite ends of their ranges for graphs with small stress and small neighborhood preservation error. See for example the properties of the two graphs from
% Figure~\ref{fig:graph-drawings}.
In this table we illustrate the top ten differences between properties of the graphs in Figure~\ref{fig:graph-drawings}
% that differ the most, 
ordered by the property values.
}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% & $\rho$ & $R_G$ & den & diam & TW & VC & TD & $C_e$ & $C_C$ & $C_B$ & $\sigma $ & ASCC & $c_4$ & $r$ & GCC &  $C_{Eig}$& NP& APL \\ \hline
% value  &0.002&0.006&0.008&0.020&0.025&0.031&0.056&0.058&0.064&0.088&0.095&0.109&0.112&0.121&0.134&0.221&0.469&0.514 \\ \hline
% \end{tabular}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
& $C_C$ & $C_B$ & $\sigma $ & ASCC & $c_4$ & $r$ & GCC &  $C_{Eig}$& NP& APL \\ \hline
value  &0.064&0.088&0.095&0.109&0.112&0.121&0.134&0.221&0.469&0.514 \\ \hline
\end{tabular}

\label{Table:graph-drawings-props}
\end{table}


==> prediction_loss_table.tex <==
 % \begin{table}[t]
% \centering
%  \caption{Prediction results for the baseline mean estimator (the first row), the linear regression estimator (the second row) and the non-linear estimator, described in Section~\ref{sec:linear_analysis}. The columns correspond to $12$ graph properties.}

% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline

%  \scalebox{0.75}[1]{$L_1$ loss}       & \scalebox{0.75}[1]{GCC}     & \scalebox{0.75}[1]{ASCC}     & \scalebox{0.75}[1]{APL}     & \scalebox{0.75}[1]{r}       & \scalebox{0.75}[1]{den}     & \scalebox{0.75}[1]{diam}    & \scalebox{0.75}[1]{Ce}      
% %  & \scalebox{0.75}[1]{Cd}
%  & \scalebox{0.75}[1]{Cc}      & \scalebox{0.75}[1]{Cb}      & \scalebox{0.75}[1]{Cei}     & \scalebox{0.75}[1]{$R_G$}     & \scalebox{0.75}[1]{$\rho$}  \\ \hline
% \scalebox{0.75}[1]{mean}     & \scalebox{0.75}[1]{.00590} & \scalebox{0.75}[1]{.00092} & \scalebox{0.75}[1]{.00017} & \scalebox{0.75}[1]{.01129} & \scalebox{0.75}[1]{.00564} & \scalebox{0.75}[1]{0}    & \scalebox{0.75}[1]{.01735} 
% % & \scalebox{0.75}[1]{.01634}
% & \scalebox{0.75}[1]{.01723} & \scalebox{0.75}[1]{.00046} & \scalebox{0.75}[1]{.00488} & \scalebox{0.75}[1]{.00578} & \scalebox{0.75}[1]{.00562} \\ \hline
% \scalebox{0.75}[1]{linear}    & \scalebox{0.75}[1]{.00099} & \scalebox{0.75}[1]{.00003} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{.00771} & \scalebox{0.75}[1]{.00002} & \scalebox{0.75}[1]{0}    & \scalebox{0.75}[1]{.01046} 
% % & \scalebox{0.75}[1]{. 00033}
%  & \scalebox{0.75}[1]{.00035} & \scalebox{0.75}[1]{.00013} & \scalebox{0.75}[1]{.00075} & \scalebox{0.75}[1]{.00006} & \scalebox{0.75}[1]{.00004 }\\ \hline
% \scalebox{0.75}[1]{non-linear} &\scalebox{0.75}[1]{.00093} & \scalebox{0.75}[1]{.00002} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{.00241} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{0}    & \scalebox{0.75}[1]{.01004} 
% %& \scalebox{0.75}[1]{ .00000*}
% & \scalebox{0.75}[1]{.00000*}
% & \scalebox{0.75}[1]{.00011} & \scalebox{0.75}[1]{.00067} & \scalebox{0.75}[1]{.00004} & \scalebox{0.75}[1]{.00001} \\ \hline
% \end{tabular}
% \vspace{-.2cm}

% \label{table:prediction_feature_old}
% \end{table}

% \begin{table}[t]
% \centering
%  \caption{Prediction results for the baseline mean estimator (the first row), the linear regression estimator (the second row) and the non-linear estimator, described in Section~\ref{sec:linear_analysis}. The columns correspond to $13$ graph properties.}

% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline

%  \scalebox{0.75}[1]{$L_1$ loss}       & \scalebox{0.75}[1]{GCC}     & \scalebox{0.75}[1]{ASCC}     & \scalebox{0.75}[1]{APL}     & \scalebox{0.75}[1]{r}       & \scalebox{0.75}[1]{diam}     & \scalebox{0.75}[1]{den}    & \scalebox{0.75}[1]{Ce}     & \scalebox{0.75}[1]{Cc}      & \scalebox{0.75}[1]{Cb}      & \scalebox{0.75}[1]{Cei}    & \scalebox{0.75}[1]{$R_G$}     & \scalebox{0.75}[1]{$\rho$} & \scalebox{0.75}[1]{TW}  \\ \hline
 
% \scalebox{0.75}[1]{mean}     & \scalebox{0.75}[1]{.00606} & \scalebox{0.75}[1]{.00095} & \scalebox{0.75}[1]{.00017} & \scalebox{0.75}[1]{.01105} & \scalebox{0.75}[1]{.00000} & \scalebox{0.75}[1]{.00597}    & \scalebox{0.75}[1]{.01756} & \scalebox{0.75}[1]{.01832} & \scalebox{0.75}[1]{.00047} & \scalebox{0.75}[1]{.00523} & \scalebox{0.75}[1]{.00613} & \scalebox{0.75}[1]{.00592} & \scalebox{0.75}[1]{.00742} \\ \hline

% \scalebox{0.75}[1]{linear}    & \scalebox{0.75}[1]{.00096} & \scalebox{0.75}[1]{.00003} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{.00733} & \scalebox{0.75}[1]{.00000} & \scalebox{0.75}[1]{.00002}    & \scalebox{0.75}[1]{.01035} & \scalebox{0.75}[1]{.00193} & \scalebox{0.75}[1]{.00013} & \scalebox{0.75}[1]{.00075} & \scalebox{0.75}[1]{.00006} & \scalebox{0.75}[1]{.00003 } & \scalebox{0.75}[1]{.00652} \\ \hline
 
% \scalebox{0.75}[1]{non-linear} &\scalebox{0.75}[1]{.00092} & \scalebox{0.75}[1]{.00002} & \scalebox{0.75}[1]{.00000*} & \scalebox{0.75}[1]{.00665} & \scalebox{0.75}[1]{.00000} & \scalebox{0.75}[1]{.00002}    & \scalebox{0.75}[1]{.01029} & \scalebox{0.75}[1]{.00183}
% & \scalebox{0.75}[1]{.00011} & \scalebox{0.75}[1]{.00067} & \scalebox{0.75}[1]{.00005} & \scalebox{0.75}[1]{.00002} & \scalebox{0.75}[1]{.00654} \\ \hline
% \end{tabular}
% \vspace{-.2cm}

% \label{table:prediction_feature_old}
% \end{table}



\begin{table}[t]
\centering
 \caption{Prediction results for the baseline mean estimator (the first row), the linear regression estimator (the second row) and the non-linear estimator, described in Section~\ref{sec:linear_analysis}. The columns correspond to $15$ graph properties.}

\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline

 \scalebox{0.75}[1]{$L_1$ loss}       & \scalebox{0.75}[1]{GCC}     & \scalebox{0.75}[1]{ASCC}     & \scalebox{0.75}[1]{APL}     & \scalebox{0.75}[1]{r}       & \scalebox{0.75}[1]{diam}     & \scalebox{0.75}[1]{den}    & \scalebox{0.75}[1]{Ce}     & \scalebox{0.75}[1]{Cc}      & \scalebox{0.75}[1]{Cb}      & \scalebox{0.75}[1]{Cei}    & \scalebox{0.75}[1]{$R_G$}     & \scalebox{0.75}[1]{$\rho$} & \scalebox{0.75}[1]{TW}  & \scalebox{0.75}[1]{TD} & \scalebox{0.75}[1]{VC} \\ \hline
 
\scalebox{0.75}[1]{mean}     & \scalebox{0.75}[1]{0.00575} & \scalebox{0.75}[1]{0.00091} & \scalebox{0.75}[1]{0.00017} & \scalebox{0.75}[1]{0.01128} & \scalebox{0.75}[1]{0.00000} & \scalebox{0.75}[1]{0.00558}    & \scalebox{0.75}[1]{0.01757} & \scalebox{0.75}[1]{0.01745} & \scalebox{0.75}[1]{0.00045} & \scalebox{0.75}[1]{0.00493} & \scalebox{0.75}[1]{0.00574} & \scalebox{0.75}[1]{0.00554} & \scalebox{0.75}[1]{0.00530} & \scalebox{0.75}[1]{0.00206} & \scalebox{0.75}[1]{0.00337} \\ \hline

\scalebox{0.75}[1]{linear}    & \scalebox{0.75}[1]{0.00093} & \scalebox{0.75}[1]{0.00003} & \scalebox{0.75}[1]{0.00000*} & \scalebox{0.75}[1]{0.00760} & \scalebox{0.75}[1]{0.00000} & \scalebox{0.75}[1]{0.00003}    & \scalebox{0.75}[1]{0.01033} & \scalebox{0.75}[1]{0.00198} & \scalebox{0.75}[1]{0.00013} & \scalebox{0.75}[1]{0.00076} & \scalebox{0.75}[1]{0.00006} & \scalebox{0.75}[1]{0.00004} & \scalebox{0.75}[1]{0.00377} & \scalebox{0.75}[1]{0.00283} & \scalebox{0.75}[1]{0.00306} \\ \hline
 
\scalebox{0.75}[1]{non-linear} &\scalebox{0.75}[1]{0.00092} & \scalebox{0.75}[1]{0.00002} & \scalebox{0.75}[1]{0.00000*} & \scalebox{0.75}[1]{0.00668} & \scalebox{0.75}[1]{0.00000} & \scalebox{0.75}[1]{0.00002} & \scalebox{0.75}[1]{0.01013} & \scalebox{0.75}[1]{0.00190} & \scalebox{0.75}[1]{0.00011} & \scalebox{0.75}[1]{0.00070} & \scalebox{0.75}[1]{0.00005} & \scalebox{0.75}[1]{0.00003} & \scalebox{0.75}[1]{0.00371} & 
\scalebox{0.75}[1]{0.00266} & \scalebox{0.75}[1]{0.00288} \\ \hline
\end{tabular}
\vspace{-.2cm}

\label{table:prediction_feature}
\end{table}





==> properties_example.tex <==
\begin{figure*}[ht]
\centering
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/4486_high_apl}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/146036_mid_apl}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/261053_low_apl}
\caption{APL is the average of the shortest paths of all pairs. As the graph in left graph has almost a path structure, degree of the vertices are very low, therefore, they are connected to few vertices. That makes the shortest paths greater(APL=0.95). So, APL value is greater for left graph. The graph in middle one has more edges, making the shortest paths a little smaller(APL=0.66). right graph has the most edges making the vertices better connected. Almost each vertex have a path of length \(1\) to another vertex. So, APL is lower than other two(APL=0.325). }
  \label{fig:apl_examples}
\end{figure*}

\begin{figure*}[ht]
\centering
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/260766_high_den}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/219525_mid_den}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/23772_low_den}
    \caption{Density is calculated by the proportion of number of present edges and  possible edges. As left graph has the highest number of edges in this figure, density value of left one is also the highest(den=0.92). The middle graph have less edges compare to left one(den=0.69). The right graph have only 10 edges(den=0.28)}
  \label{fig:den_examples}
\end{figure*}

\begin{figure*}[ht]
\centering
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/64550_high_diam}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/23020_mid_diam}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/261079_low_diam}
\caption{We are showing the normalized diameter here. Diameter is the longest shortest paths of the vertex-pairs. left graph has the longest shortest path \(7\)(diam=0.875, after normalized). The middle graph has the longest shortest path \(4\)(diam=0.5) while right graph has longest shortest path \(1\)(diam=0.125).}
  \label{fig:diam_examples}
\end{figure*}

\begin{figure*}[ht]
    \includegraphics[width=0.3\textwidth]{./figures/prop_examples/high_r}
    \includegraphics[width=0.2\textwidth,angle=90]{./figures/prop_examples/medium_r}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/29_high_r}
    \caption{The left graph have $r=0.81$, middle one have $r=0$ and the right one have $r=0.98$ In left graph, most of the vertices are connected to vertices with similar degree values. The right graph is opposite. The low-degree vertices are connected to high-degree vertices. Therefore, these two have these two extreme values. On the other hand, the one in the middle does not create any community of high-degree and low-degree vertices. All of the vertices have very close degree value. So, degree assortativity is \(0\). }
  \label{fig:r_examples}
\end{figure*}

\begin{figure*}[ht]
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/261077_high_ce}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/256444_mid_ce}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/256537_low_ce}
    \caption{The left graph have $C_E = 0.87$, middle one have$C_E = 0.62$ and right one have $C_E = 0.12$. as shown in graph, with higher $C_E$, the graph are more connected and hard to disconnected. In the right graph, we can easily  disconnected the graph by removing only one edge. Therefore, edge connectivity is small.}
  \label{fig:ce_examples}
\end{figure*}

\begin{figure*}[ht]
\includegraphics[width=0.3\textwidth]{./figures/prop_examples/7_high_degree}
\includegraphics[width=0.3\textwidth]{./figures/prop_examples/mid_degree.pdf}
\includegraphics[width=0.3\textwidth]{./figures/prop_examples/low_degree1.pdf}
\caption{$C_D$ for left, middle and right graphs is $0.93, 0.5, 0.13$, respectively. left and middle graphs both has one high-degree vertices. the high-degree vertices in left graph is connected to all of the vertices and all other vertices have only small degrees. The middle graph have several vertices that have degree more than $4$, Therefore the  $C_D$ for it is not as high as left one.  vertices in the right graph almost have  similar degrees. So, $C_D$ is small.}
  \label{fig:dc_examples}
\end{figure*}

\begin{figure*}[ht]
    \includegraphics[width=0.3\textwidth,angle=90]{./figures/prop_examples/37_high_cc}
    \includegraphics[width=0.3\textwidth,angle=90]{./figures/prop_examples/257115_mid_cc}
    \includegraphics[width=0.3\textwidth,angle=90]{./figures/prop_examples/248698_low_cc}
    \caption{$C_c$ for left, middle and right graphs is $0.96, 0.47, ~0$, respectively. left and middle graphs both have high-degree vertices. the only high-degree vertices in left graph is connected to most of the vertices and all other vertices have only small degrees. Most vertices in middle graph have high degree. Therefore the correlation for it is not as high as left one. vertices in the right graph are far from each other.}
  \label{fig:cc_examples}
\end{figure*}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[ht]
    \includegraphics[width=0.3\textwidth,angle=90]{./figures/prop_examples/2_high_between}
    \includegraphics[width=0.3\textwidth,angle=90]{./figures/prop_examples/256550_mid_between}
\includegraphics[width=0.3\textwidth]{./figures/prop_examples/low_between}
  \caption{$C_B$ for left, middle and right graphs is $0.96, 0.52, 0.06$, respectively. }
  \label{fig:bet_examples}
\end{figure*}

\begin{figure*}[ht]
    \includegraphics[width=0.31\textwidth,angle=90]{./figures/prop_examples/35_high_eigen}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/4551_mid_eigen}
    \includegraphics[width=0.35\textwidth,angle=90]{./figures/prop_examples/256483_low_eigen}
    \caption{$C_{ei}$ for left, middle and right graphs is $0.95, 0.49, ~0$, respectively.}
  \label{fig:cei_examples}
\end{figure*}

% \begin{figure*}[h]
% \centering
% \begin{subfigure}{\dis\textwidth}
%     \centering
%     \includegraphics[width=0.7\textwidth,angle=90]{./figures/prop_examples/261078_high_egr}
%     \caption{A graph with $|V|=9, |E|=35, E\_G\_resist=0.965517241 $ }
%     \label{fig:high_egr}
% \end{subfigure}
% \begin{subfigure}{\dis\textwidth}
%     \centering
%     \includegraphics[width=0.7\textwidth,angle=90]{./figures/prop_examples/195985_mid_egr}
%     \caption{A graph with $|V|=9, |E|=26, E\_G\_resist=0.630631 $ }
%     \label{fig:mid_egr}
% \end{subfigure}
% \begin{subfigure}{\dis\textwidth}
%     \centering
%     \includegraphics[width=0.7\textwidth,angle=90]{./figures/prop_examples/146067_low_egr}
%     \caption{A graph with $|V|=9, |E|=16, E\_G\_resist=0.263158 $ }
%     \label{fig:low_egr}
%     \end{subfigure}
%     \caption{Graphs with high, medium and low-valued effective graph resistance.}
%   \label{fig:egr_examples}
% \end{figure*}

% \begin{figure*}[h]
% \centering
% \begin{subfigure}{\dis\textwidth}
%     \centering
%     \includegraphics[width=0.7\textwidth,angle=90]{./figures/prop_examples/261054_high_sr}
%     \caption{A graph with $|V|=9, |E|=34, S_{rad}=0.950694 $ }
%     \label{fig:high_sr}
% \end{subfigure}
% \begin{subfigure}{\dis\textwidth}
%     \centering
%     \includegraphics[width=0.7\textwidth,angle=90]{./figures/prop_examples/22649_mid_sr}
%     \caption{A graph with $|V|=9, |E|=15, S_{rad}=0.503142969 $ }
%     \label{fig:mid_sr}
% \end{subfigure}
% \begin{subfigure}{\dis\textwidth}
%     \centering
%     \includegraphics[width=0.7\textwidth,angle=90]{./figures/prop_examples/24344_low_sr}
%     \caption{A graph with $|V|=9, |E|=8, S_{rad}=0.237764 $ }
%     \label{fig:low_sr}
%     \end{subfigure}
%     \caption{Graphs with high, medium and low-valued spectral radius. Spectral radius shows us the relation of average degree and the highest degree in the graph. For any graph with specific number of vertices, the range of spectral radius is from average degree to the highest degree in that graph. The first graph here has an average of around 7.5 degree which will be around 0.94 if normalized. The highest degree in this graph is 8, i.e; 1 as normalized. The graph is (b), however has a lower average, 0.42 as normalized. The last graph has 0.22 as average and 0.25 as highest degree. We can see that all of the spectral radius is in this range. }
%     % https://www.epfl.ch/labs/dcg/wp-content/uploads/2018/10/ADM-Eigenvalues-v3.pdf
%   \label{fig:sr_examples}
% \end{figure*}


==> same_stat.tex <==
\begin{figure}[t]
	\includegraphics[width=.24\textwidth]{./figures/same_stat/same_stat_v=100_1}
	\includegraphics[width=.24\textwidth]{./figures/same_stat/same_stat_v=100_2}
	\includegraphics[width=.24\textwidth]{./figures/same_stat/same_stat_v=100_3}
	\includegraphics[width=.24\textwidth]{./figures/same_stat/same_stat_v=100_4}

	\caption{ Four graphs generated by the \ErdosRenyi model with $p=1/2$ and $|V|=100$, with the same 12 properties (up to 2 decimal places). In $1000$  generated graphs, on average there are 78 pairs, 15 triples and 3 quadruples with the same 12 properties. Note that the graphs are not isomorphic to each other.}
	%since they have different degree sequences.}
	\label{fig:same_stat_4_tuple}
	\centering
\end{figure}
% \todo{remove this figure?}
